NASA: Neural Architecture Search and Acceleration for Hardware Inspired Hybrid Networks

Multiplication is arguably the most cost-dominant operation in modern deep neural networks (DNNs), limiting their achievable efficiency and thus more extensive deployment in resource-constrained applications. To tackle this limitation, pioneering works have developed handcrafted multiplication-free DNNs, which require expert knowledge and time-consuming manual iteration, calling for fast development tools. To this end, we propose a Neural Architecture Search and Acceleration framework dubbed NASA, which enables automated multiplication-reduced DNN development and integrates a dedicated multiplication-reduced accelerator for boosting DNNs' achievable efficiency. Specifically, NASA adopts neural architecture search (NAS) spaces that augment the state-of-the-art one with hardware-inspired multiplication-free operators, such as shift and adder, armed with a novel progressive pretrain strategy (PGP) together with customized training recipes to automatically search for optimal multiplication-reduced DNNs; On top of that, NASA further develops a dedicated accelerator, which advocates a chunk-based template and auto-mapper dedicated for NASA-NAS resulting DNNs to better leverage their algorithmic properties for boosting hardware efficiency. Experimental results and ablation studies consistently validate the advantages of NASA's algorithm-hardware co-design framework in terms of achievable accuracy and efficiency tradeoffs. Codes are available at https://github.com/GATECH-EIC/NASA.

==> section/2-Preliminary.tex <==
\section{Preliminary}
In this section, we discuss shift layers in \cite{DeepShift}, adder layers in \cite{AdderNet}, and shiftadd layers in \cite{ShiftAddNet} mathematically and explicitly, which inspire the formation of our novel search spaces. The differentiation and affiliation of vanilla convolutions and these multiplication-less operations are described in Fig. \ref{operator_fig}. 

% \vspace{-1em}
\begin{figure}[htbp]
	\centerline{\includegraphics[width=3.7in]{Operations.pdf}}
	\caption{The overview of $(a)$ traditional convolutions, $(b)$ shift layers, $(c)$ adder layers, and $(d)$ shiftadd layers.
	As we can see, convolution layer conducts extensive multiplications, shift layer adopts bitwise shift and sign flipping instead, adder layer contains only additions, and shiftadd layer is composed of a shift layer and an adder layer.}
	\label{operator_fig}
\end{figure}
% \vspace{-1em}

% \begin{table}[htbp]
% 	\centering
% 	\caption{The Parameter Number and FLOPs Compression between the Image Transform Net and MobileNet}
% 	\begin{threeparttable}
% 	\begin{tabular}{|c|c|c|}
% 	\hline
% 	Model            & Image Transform Net & MobileNet \\ \hline
% 	Parameter Number & 1.68 M              & 4.2 M       \\ \hline
% 	FLOPs \tnote{1}  & 15.48 G             & 1.00 G       \\ \hline
%     \end{tabular}
% 	 \end{threeparttable}
% 	\label{related_work}
% \end{table}
% \begin{table}[]
% 	\centering
% 	\caption{The comparison of energy and area between multiply, add, and shift. }
% 	\begin{tabular}{cc|cccc}
% 	\hline
% 	\multicolumn{2}{c|}{Operator}                                   & \multicolumn{4}{c}{ASIC}                                     \\ \hline
% 	Oprator & Format                                                & Energy(pJ) & \multicolumn{1}{c|}{Improved} & Area & Improved \\ \hline
% 	Multiply & \begin{tabular}[c]{@{}c@{}}FP32\\ INT16\end{tabular}  &            & \multicolumn{1}{c|}{}         &      &          \\ \hline
% 	Add     & \begin{tabular}[c]{@{}c@{}}FP32\\ INT16\end{tabular}  &            & \multicolumn{1}{c|}{}         &      &          \\ \hline
% 	Shift   & \begin{tabular}[c]{@{}c@{}}INT32\\ INT16\end{tabular} &            & \multicolumn{1}{c|}{}         &      &          \\ \hline
% 	\end{tabular} \label{operators}
% 	\end{table}

\subsection{Shift Layers}
\label{sec:shift_layer}
Bitwise shift operations are energy efficient and popularly used in hardware designs, which are equivalent to multiplying or dividing by powers of two. 
% As proofed in Table \ref{operators}, the bitwise shift can realize to energy saving and to area reduction when compared with multiplications. 
DeepShift \cite{DeepShift} generated shift layers by adopting bitwise shift ${p}$ combined with sign flipping ${s}$ to replace multiplications in filters, which is shown in Fig. \ref{operator_fig} and expressed as: 
\begin{equation}
	% \begin{aligned}
	% \textbf{Y}(m,n,t) = \sum_{i = 0}^{d}\sum_{j = 0}^{d}\sum_{k = 0}^{c_{in}}(\textbf{x}(m+i,n+j,k)*\textbf{w}(i,j,k,t)), 
	% \\w = s*2^{p}, where \hfill \label{shift}
	% \end{aligned}
	\begin{aligned}
		Y_{s}(m,n,t) = \sum_{i = 0}^{d}&\sum_{j = 0}^{d}\sum_{k = 0}^{c_{in}}(x_{s}(m+i,n+j,k)*w_{ps}(i,j,k,t)), 
		\\&w_{ps} = s*2^{p}, where \hfill 
		\end{aligned} \label{shift_weight}
\end{equation}

\begin{equation}
2^p*x=\left\{
\begin{array}{lcl}
x<<p       &    if\ {p > 0}\\
x>>p       &     if \ {p < 0}\\
x          &    if \ {p = 0}\\
\end{array}\right.
s*x=\left\{
\begin{array}{lll}
	+x       &    if \ {s = 1}\\
	0       &     if\ {s=0}\\
	-x          &    if \ {s = -1} \\
	
	\end{array} \right.
\end{equation}

$Y_{s}$, $x_{s}$, and $w_{ps}$ donate the outputs, inputs, and weights of shift layers, respectively. $m$, $n$, and $t$ represent the position of row, column, and channel in output feature maps. $d$ and $c_{in}$ stand for the kernel size and number of input channels in weights, respectively. $p$ determines the bit number of shift, which is always negative in \cite{DeepShift}. $s$ implements sign flipping for the positive $2^p$.

By approximately using a straight through estimator (STE) \cite{yin2019understanding}, i.e., $\partial{sign(x)}=\partial{x}$, following \cite{DeepShift}, the backpropagation of shift layers can be represented as:
\begin{equation}
	% \mathbf{\frac{\partial{Y}}{\partial{p}} = \frac{\partial{Y}}{\partial{Y_{s}}}\frac{\partial{Y_{s}}}{\partial{w_{s}}}{w_{s}}ln2}, \quad\mathbf{\frac{\partial{Y}}{\partial{s}} = \frac{\partial{Y}}{\partial{Y_{s}}}\frac{\partial{Y_{s}}}{\partial{w_{s}}}}, \quad\mathbf{\frac{\partial{Y}}{\partial{x}} = \frac{\partial{Y}}{\partial{Y_{s}}}\mathbf{w_{s}}^\mathrm{T}}
	\frac{\partial{Y_{s}}}{\partial{p}} = \frac{\partial{Y_{s}}}{\partial{w_{ps}}}w_{ps}\cdot{ln2}, \quad\frac{\partial{Y_{s}}}{\partial{s}} = \frac{\partial{Y_{s}}}{\partial{w_{ps}}},
	\quad \frac{\partial{Y_{s}}}{\partial{x_{s}}} = \mathrm{w_{ps}}^\mathrm{T}. \label{shift}
\end{equation}


\subsection{Adder Layers}
% The multiplication-intensive convolutions in DNNs are essentially cross correlation fuctions to measure the 
% relevance between input and output activations.
From the mathematical perspective, the multiplication-intensive convolutions in DNNs are essentially cross-correlation functions used to measure the relevance between input activations and weights.
%  AdderNet \cite{AdderNet} took the $\ell1$-norm distance between inputs and filters as output response to measure the similarity
% As listed in Table \ref{operators} , add can achieve   to  energy saving and  to  area reduction when compared with multiplications. 
To utilize the superiority of add operations, AdderNet \cite{AdderNet} proposed adder layers, and took the $\ell1$-norm distance between inputs and filters as the output response instead to measure the similarity, as shown in Fig. \ref{operator_fig} and expressed as:
\begin{equation}
	\begin{aligned}
		Y_{a}(m,n,t) =& -\sum_{i = 0}^{d}\sum_{j = 0}^{d}\sum_{k = 0}^{c_{in}}\\& \left\lvert(x_{a}(m+i,n+j,k) -w_{a}(i,j,k,t))\right\rvert.
		\end{aligned} 
\end{equation} 
Where $Y_{a}$, $x_{a}$, and $w_{a}$ donate the outputs, inputs, and weights of adder layers, respectively, and the definitions of $m$, $n$, $t$, $d$ and $c_{in}$ are the same to Eq. \ref{shift}.

Considering that signSGD \cite{signSGDCO} is not suitable for DNN optimization, \cite{AdderNet} treated $sign(x)=x$ during backpropagation. The partial derivative of outputs $Y_{a}$ with respect to weights $w_{a}$ is calculated as:
\begin{equation}
	\frac{\partial{Y_{a}(m,n,t)}}{\partial{w_{a}(i,j,k,t)}} = x_{a}(m+i,n+j,k)-w(i,j,k,t). \label{adder_bp_w}
\end{equation}  

To prevent gradient explosion, the gradient of $x_{a}$ is clipped to $[-1,1]$ and expressed as:
\begin{equation}
	\frac{\partial{Y_{a}(m,n,t)}}{\partial{x_{a}(m+i,n+j,k)}} = HT(w_{a}(i,j,k,t)-x_{a}(m+i,n+j,k)), \label{adder_bp_x}
\end{equation}
where $HT(\cdot)$ represents the HardTanh function.
% \begin{equation}
% 	HT(x)=\left\{
% 	\begin{array}{lcl}
% 	x       &    if  & {-1 < x < 1}\\
% 	1       &     if & {x > 1}\\
% 	-1          &    if  & {x < -1}\\
% 	\end{array}\right.
% 	\end{equation}


\subsection{Shiftadd layers}
From hardware perspective, bitwise shifts and additions are widely used as equivalent substitutes for multiplications to reduce computational cost and complexity. From algorithmic perspective, shift layers are produced to abstract coarse-grained features, while adder layers are created to extract fine-grained features. To improve the expressive capacity of multiplication-less networks, ShiftAddNet \cite{ShiftAddNet} integrated the two weaker players (shift layer and adder layer) together to form shiftadd layer, which are explained in Fig. \ref{operator_fig} and formulated as follows:
\begin{equation}
\begin{aligned}
		Y_{sa}=k_{a}(k_{s}(x_{s},s\cdot2^{p}),w_{a})&,where 
		\\k_{s}(x_{s},w_{s})=\sum \mathbf{x_{s}}^\mathrm{T}*w_{s} ,\\
		k_{a}(x_{a},w_{a})=-\sum|w_{a}-x_{a}| .
		\end{aligned}
\end{equation} 
$Y_{sa}$ donates output activations of shiftadd layers, $k_{a}(\cdot,\cdot)$ and $k_{s}(\cdot,\cdot)$ are kernel functions of adder layers and shift layers, respectively. A shiftadd layer with the shape of $(k, k, c_{in}, c_{out}, s, p)$ contains a $(k, k, c_{in}, c_{out}, s, p)$ shift layer and a $(k, k, c_{out}, c_{out}, $1$, p)$ adder layer, where $k$ is the kernel size, $c_{in}$, $c_{out}$, $s$ and $p$ donate the input and output channel dimensions,
stride number, and padding size, respectively.

The backpropagation of add layer in shiftadd layer follows Eq. (\ref{adder_bp_w}) and Eq. (\ref{adder_bp_x}),
while the backpropagation of shift layer is reformulated as:
% the difference is Eq. (\ref{shift}) in shift layer, which is reformulated as:
% \begin{small}
\begin{equation}
\begin{aligned}
 	\frac{\partial{Y_{sa}}}{\partial{p}} = \frac{\partial{Y_{sa}}}{\partial{Y_{s}}}\frac{\partial{Y_{s}}}{\partial{w_{s}}}w_{s}\cdot{ln2},
 	\quad\frac{\partial{Y_{sa}}}{\partial{s}} =& \frac{\partial{Y_{sa}}}{\partial{Y_{s}}}\frac{\partial{Y_{s}}}{\partial{w_{s}}},\\
	\frac{\partial{Y_{sa}}}{\partial{x_{s}}} = \frac{\partial{Y_{sa}}}{\partial{Y_{s}}}\mathbf{w_{s}}^\mathrm{T}.   
\end{aligned}
\end{equation}
% \end{small}
% The definitions of $p$, 

==> section/Abstract.tex <==
\begin{abstract}
% 	Multiplication is arguably the most cost-dominant operation in modern deep neural networks (DNNs), limiting their achievable efficiency and thus more extensive deployment into resource-constrained applications. To tackle this limitation, pioneering works have developed handcrafted multiplication-less DNNs, which require expert knowledge and time-consuming manual iteration, calling for fast development tools. To this end, we propose NASA (neural architecture search and acceleration framework), which enables automated multiplication-less DNN development and integrates dedicated multiplication-less accelerators for boosted DNN efficiency. Specifically, NASA adopts a neural architecture search (NAS) space that augments state-of-the-art ones with hardware inspired multiplication-less operators, such as shift and add, and a differentiable NAS search algorithm to automatically search for multiplication-less DNNs; On top of that, NASA further develops a dedicated accelerator for the NASA-NAS resulting DNNs to better leverage their algorithmic properties for boosting hardware efficiency. Experimental results and ablation studies validate the advantages of our proposed NASA algorithm-hardware co-design framework in terms of achieved accuracy and efficiency. All the codes will be released publicly upon acceptance.

Multiplication is arguably the most cost-dominant operation in deep neural networks (DNNs), limiting their achievable efficiency and thus more extensive applications into resource-constrained devices. As such, pioneering works have developed handcrafted multiplication-less DNNs, which require expert knowledge and time-consuming manual iteration, calling for fast development tools. To this end, we propose NASA (a Neural Architecture Search and Acceleration framework), which enables automated hybrid DNN development and integrates dedicated accelerators to better leverage hybrid DNNs’ algorithmic properties for boosted hardware efficiency. Extensive experiments validate the advantages of our proposed NASA algorithm-hardware co-design framework in terms of achieved accuracy and efficiency. 
\end{abstract}
